Automatic partitioning for the low-rank integration of stochastic Boolean reaction networks

Boolean reaction networks are an important tool in biochemistry for studying mechanisms in the biological cell. However, the stochastic formulation of such networks requires the solution of a master equation which inherently suffers from the curse of dimensionality. In the past, the dynamical low-rank (DLR) approximation has been repeatedly used to solve high-dimensional reaction networks by separating the network into smaller partitions. However, the partitioning of these networks was so far only done by hand. In this paper, we present a heuristic, automatic partitioning scheme based on two ingredients: the Kernighan-Lin algorithm and information entropy. Our approach is computationally inexpensive and can be easily incorporated as a preprocessing step into the existing simulation workflow. We test our scheme by partitioning Boolean reaction networks on a single level and also in a hierarchical fashion with tree tensor networks. The resulting accuracy of the scheme is superior to both partitionings chosen by human experts and those found by simply minimizing the number of reaction pathways between partitions.

==> bibliography.tex <==
@article{Albeck_2008,
    author = {Albeck, J. G. and Burke, J. M. and Spencer, S. L. and Lauffenburger, D. A. and Sorger, P. K.},
    doi = {10.1371/journal.pbio.0060299},
    journal = {PLOS Biol.},
    volume = {12},
    number = {6},
    pages = {2831--2852},
    title = {{Modeling a Snap-Action, Variable-Delay Switch Controlling Extrinsic Cell Death}},
    year = {2008}
}

@article{Albi_2022,
    author = {Albi, G. and Chignola, R. and Ferrarese, F.},
    doi = {10.1016/j.matcom.2022.03.019},
    journal = {Math. Comput. Simul.},
    volume = {199},
    pages = {317--340},
    title = {{Efficient ensemble stochastic algorithms for agent-based models with spatial predator--prey dynamics}},
    year = {2022}
}

@article{Anderson_2010,
    author = {Anderson, D. F.},
    doi = {10.1007/s11538-010-9517-4},
    journal = {Bulletin of Mathematical Biology},
    volume = {72},
    pages = {1947--1970},
    title = {{Product-Form Stationary Distributions for Deficiency Zero Chemical Reaction Networks}},
    year = {2010}
}

@article{Arnold_2013,
    author = {Arnold, A. and Jahnke, T.},
    doi = {10.1007/s10543-013-0444-2},
    journal = {BIT Numer. Math.},
    volume = {54},
    pages = {305--341},
    title = {{On the approximation of high-dimensional differential equations in the hierarchical Tucker format}},
    year = {2013}
}

@article{Allmann-Rahn_2022,
    author = {Allmann-Rahn, F. and Grauer, R. and Kormann, K.},
    doi = {10.1016/j.jcp.2022.111562},
    journal = {J. Comput. Phys.},
    volume = {469},
    pages = {111562},
    title = {{A parallel low-rank solver for the six-dimensional Vlasov--Maxwell equations}},
    year = {2022},
}

@article{Bachmayr_2023,
    author = {Bachmayr, M.},
    doi = {10.1017/S0962492922000125},
    journal = {Acta Numer.},
    volume = {32},
    pages = {1--121},
    title = {{Low-rank tensor methods for partial differential equations}},
    year = {2023},
}

@article{Barabasi_2009,
    author = {Barab\'{a}si, A.-L.},
    doi = {10.1126/science.1173299},
    journal = {Science},
    volume = {325},
    number = {5939},
    pages = {412--413},
    title = {{Scale-Free Networks: A Decade and Beyond}},
    year = {2009},
}

@article{Barbuti_2020,
    author = {Barbuti, R. and Gori, R. and Milazzo, P. and Nasti, L.},
    doi = {10.1007/s41965-020-00046-y},
    journal = {J. Membr. Comput.},
    volume = {2},
    pages = {207--226},
    title = {{A survey of gene regulatory networks modelling methods:
from differential equations, to Boolean and qualitative bioinspired models}},
    year = {2020},
}

@article{Benso_2014,
    author = {Benso, A. and Di Carlo, S. and Politano, G. and Savino, A. and Vasciaveo, A.},
    doi = {10.1186/1742-4682-11-S1-S5},
    journal = {Theor. Biol. Med. Model.},
    volume = {11},
    number = {S5},
    title = {An extended gene protein/products boolean network model including post-transcriptional regulation},
    year = {2014},
}

@article{Cai_2017,
    author = {Cai, X. and Guo, W. and Qiu, J.-M.},
    doi = {10.1007/s10915-017-0554-0},
    journal = {J. Sci. Comput.},
    volume = {73},
    title = {{A high order conservative semi-Lagrangian discontinuous Galerkin method for two-dimensional transport simulations}},
    year = {2017}
}

@article{Calzone_2010,
    author = {Calzone, L. and Tournier, L. and Fourquet, S. and Thieffry, D. and Zhivotovsky, B. and Barillot, E. and Zinovyev, A.},
    doi = {10.1371/journal.pcbi.1000702},
    journal = {PLOS Comput. Biol.},
    volume = {6},
    number = {3},
    title = {{Mathematical Modelling of Cell-Fate Decision in Response to Death Receptor Engagement}},
    year = {2010}
}

@article{Cassini_2021,
    author = {Cassini, F. and Einkemmer, L.},
    doi = {10.1016/j.cpc.2022.108489},
    journal = {Comput. Phys. Commun.},
    volume = {280},
    title = {{Efficient 6D Vlasov simulation using the dynamical low-rank framework \texttt{Ensign}}},
    year = {2022}
}

@article{Ceruti_2020,
    author = {Ceruti, G. and Lubich, C. and Walach, H.},
    doi = {10.1137/20M1321838},
    journal = {SIAM J. Numer. Anal.},
    volume = {59},
    number = {1},
    pages = {289--313},
    title = {Time integration of tree tensor networks},
    year = {2021},
}

@article{Ceruti_2022,
    author = {Ceruti, G. and Lubich, C.},
    doi = {10.1007/s10543-021-00873-0},
    journal = {BIT Numer. Math.},
    volume = {62},
    number = {1},
    pages = {23--44},
    title = {{An unconventional robust integrator for dynamical low-rank approximation}},
    year = {2022}
}

@article{Ceruti_2022a,
    author = {Ceruti, G. and Kusch, J. and Lubich, C.},
    doi = {10.1007/s10543-021-00907-7},
    journal = {BIT Numer. Math.},
    volume = {62},
    pages = {1149--1174},
    title = {{A rank-adaptive robust integrator for dynamical low-rank approximation}},
    year = {2022},
}

@article{Ceruti_2023,
    author = {Ceruti, G. and Lubich, C. and Sulz, D.},
    doi = {10.1137/22M1473790},
    journal = {SIAM J. Numer. Anal.},
    volume = {61},
    number = {1},
    pages = {194--222},
    title = {{Rank-adaptive time integration of tree tensor networks}},
    year = {2023}
}

@article{Ceruti_2024,
    author = {Ceruti, G. and Kressner, D. and Sulz, D.},
    doi = {10.48550/arXiv.2405.09952},
    journal = {arXiv},
    title = {{Low-rank Tree Tensor Network Operators for Long-Range Pairwise Interactions}},
    year = {2024}
}

@article{Ceruti_2024a,
    author = {Ceruti, G. and Kusch, J. and Lubich, C.},
    doi = {10.1137/23M1565103},
    journal = {SIAM J. Sci. Comput.},
    volume = {46},
    number = {3},
    pages = {B205--B228},
    title = {{A parallel rank-adaptive integrator for dynamical low-rank approximation}},
    year = {2024}
}

@article{Ceruti_2024b,
    author = {Ceruti, G. and Einkemmer, L. and Kusch, J. and Lubich, C.},
    doi = {10.1007/s10543-024-01032-x},
    journal = {BIT Numer. Math.},
     volume = {64},
    number = {30},
    title = {{A robust second-order low-rank BUG integrator based on the midpoint rule}},
    year = {2024}
}

@article{Ceruti_2024c,
    author = {Ceruti, G. and Kusch, J. and Lubich, C. and Sulz, D.},
    doi = {10.48550/arXiv.2412.00858},
    journal = {arXiv},
    title = {{A parallel Basis Update and Galerkin integrator for tree tensor networks}},
    year = {2024}
}

@article{Chen_2010,
    author = {Chen, W. W. and Niepel, M. A. and Sorger, P. K.},
    doi = {10.1101/gad.1945410},
    journal = {Genes Dev.},
    volume = {24},
    number = {17},
    pages = {1861--1875},
    title = {{Classic and contemporary approaches to modeling biochemical reactions}},
    year = {2010}
}

@article{Clarke_2020,
    author = {Clarke, M. A. and Fisher, J.},
    doi = {10.1038/s41568-020-0258-x},
    journal = {Nat. Rev. Cancer},
    volume = {20},
    pages = {343--354},
    title = {{Executable cancer models: successes and challenges}},
    year = {2020}
}

@article{Coughlin_2022,
    author = {Coughlin, J. and Hu, J.},
    doi = {10.1016/j.jcp.2022.111590},
    journal = {J. Comput. Phys.},
    volume = {470},
    pages = {111590},
    title = {{Efficient dynamical low-rank approximation for the Vlasov-Amp\`{e}re-Fokker-Planck system}},
    year = {2022},
}

@article{Coughlin_2024,
    author = {Coughlin, J. and Hu, J. and Shumlak, U.},
    doi = {10.1016/j.jcp.2024.113055},
    journal = {J. Comput. Phys.},
    volume = {509},
    pages = {113055},
    title = {{Robust and conservative dynamical low-rank methods for the Vlasov equation via a novel macro-micro decomposition}},
    year = {2024},
}

@article{Ding_2021,
    author = {Ding, Z. and Einkemmer, L. and Li, Q.},
    doi = {10.1137/20M1380788},
    journal = {SIAM J. Numer. Anal.},
    volume = {59},
    number = {4},
    title = {{Dynamical Low-Rank Integrator for the Linear Boltzmann Equation: Error Analysis in the Diffusion Limit}},
    year = {2021}
}

@article{Dinh_2020,
    author = {Dinh, T. and Sidje, R. B.},
    doi = {10.1088/1478-3975/aba1d2},
    journal = {Phys. Biol.},
    volume = {17},
    number = {065014},
    title = {{An adaptive solution to the chemical master equation using quantized tensor trains with sliding windows}},
    year = {2020}
}

@article{Dolgov_2015,
    author = {Dolgov, S. and Khoromskij, B.},
    doi = {10.1002/nla.1942},
    journal = {Numer. Linear Algebra Appl.},
    volume = {22},
    pages = {197--219},
    title = {{Simultaneous state-time approximation of the chemical master equation using tensor product formats}},
    year = {2015}
}

@article{Einkemmer_2018,
    author = {Einkemmer, L. and Lubich, C.},
    doi = {10.1137/18M116383X},
    journal = {SIAM J. Sci. Comput.},
    volume = {40},
    number = {5},
    pages = {B1330--B1360},
    title = {{A Low-Rank Projector-Splitting Integrator for the Vlasov-Poisson Equation}},
    year = {2018}
}

@article{Einkemmer_2020,
    author = {Einkemmer, L. and Ostermann, A. and Piazzola, C.},
    journal = {J. Comput. Phys.},
    volume = {403},
    pages = {109063},
    title = {{A low-rank projector-splitting integrator for the Vlasov--Maxwell equations with divergence correction}},
    year = {2020}
}

@article{Einkemmer_2021,
    author = {Einkemmer, L. and Hu, J. and Wang, Y.},
    doi = {10.1016/j.jcp.2021.110353},
    journal = {J. Comput. Phys.},
    volume = {439},
    number = {110353},
    pages = {110353},
    title = {{An asymptotic-preserving dynamical low-rank method for the multi-scale multi-dimensional linear transport equation}},
    year = {2021}
}

@article{Einkemmer_2021a,
    author = {Einkemmer, L. and Hu, J. and Ying, L.},
    doi = {10.1137/21m1392772},
    journal = {SIAM J. Sci. Comput.},
    volume = {43},
    number = {5},
    pages = {B1057--B1080},
    title = {{An Efficient Dynamical Low-Rank Algorithm for the Boltzmann-{BGK} Equation Close to the Compressible Viscous Flow Regime}},
    year = {2021}
}

@article{Einkemmer_2021b,
    author = {Einkemmer, L. and Joseph, I.},
    doi = {10.1016/j.jcp.2021.110495},
    journal = {J. Comput. Phys.},
    volume = {443},
    pages = {110495},
    title = {{A mass, momentum, and energy conservative dynamical low-rank scheme for the Vlasov equation}},
    year = {2021}
}

@misc{Einkemmer_2021c,
    author = {Einkemmer, L.},
    title = {{Lecture slides: Low-rank approximation for nonlinear kinetic problems -- Part 1: Introduction and the dynamical low-rank algorithm}},
    year = {2021}
}

@article{Einkemmer_2022,
    author = {Einkemmer, L. and Ostermann, A. and Scalone, C.},
    doi = {10.1016/j.jcp.2023.112060},
    journal = {J. Comput. Phys.},
    volume = {484},
    pages = {112060},
    title = {A robust and conservative dynamical low-rank algorithm},
    year = {2023}
}

@article{Einkemmer_2023,
    author = {Einkemmer, L.},
    doi = {10.1016/j.jcp.2024.112757},
    journal = {J. Comput. Phys.},
    volume = {501},
    number = {112757},
    title = {{Accelerating the simulation of kinetic shear Alfv\'{e}n waves with a dynamical low-rank approximation}},
    year = {2024}
}

@article{Einkemmer_2024,
    author = {Einkemmer, L. and Mangott, J. and Prugger, M.},
    doi = {10.1016/j.jcp.2024.112827},
    journal = {J. Comput. Phys.},
    volume = {503},
    number = {112827},
    title = {{A low-rank complexity reduction algorithm for the high-dimensional kinetic chemical master equation}},
    year = {2024}
}

@article{Einkemmer_2024a,
    author = {Einkemmer, L. and Hu, J. and Kusch, J.},
    doi = {10.1137/23M1547603},
    journal = {SIAM J. Numer. Anal.},
    volume = {62},
    number = {1},
    pages = {73--92},
    title = {Asymptotic--preserving and energy stable dynamical low-rank approximation},
    year = {2024}
}

@article{Einkemmer_2024b,
    author = {Einkemmer, L. and Mangott, J. and Prugger, M.},
    doi = {10.48550/arXiv.2407.11792},
    journal = {arXiv},
    title = {{A hierarchical dynamical low-rank algorithm for the stochastic description of large reaction networks}},
    year = {2024}
}

@online{Einkemmer_2024c,
    author = {Einkemmer, L. and Mangott, J. and Prugger, M.},
    title = {\textup{\texttt{hierarchical-cme}}},
    year = {2024},
    url = {https://github.com/jmangott/hierarchical-cme/tree/boolean}
}

@InProceedings{Ellson_2001,
    author = {Ellson, J. and Gansner, E. and Koutsofios, L. and North, S. C. and Woodhull, G.},
    editor = {Mutzel, P. and J\"{u}nger, M. and Leipert, S.},
    pages = {483–484},
    series = {LNCS 2265},
    booktitle = {{Graph Drawing (GD 2001)}},
    title = {{\texttt{Graphviz} -- Open Source Graph Drawing Tools}},
    year = {2001},
    publisher = {Springer}
}


@article{Engblom_2008,
    author = {Engblom, S.},
    doi = {10.1016/j.cam.2008.10.029},
    journal = {J. Comput. Appl. Math.},
    volume = {229},
    pages = {208--221},
    title = {{Spectral approximation of solutions to the chemical master equation}},
    year = {2008}
}

@book{Erban_2020,
    author = {Erban, R. and Chapman, S. J.},
    doi = {10.1017/9781108628389},
    publisher = {Cambridge University Press},
    title = {{Stochastic Modelling of Reaction--Diffusion Processes}},
    year = {2020}
}

@article{Faure_2006,
    author = {Faur\'{e}, A. and Naldi, A. and Chaouiya, C. and Thieffry, D.},
    doi = {10.1093/bioinformatics/btl210},
    journal = {Bioinformatics},
    volume = {22},
    number = {14},
    pages = {e124--e131},
    title = {{Dynamical analysis of a generic Boolean model for the control of the mammalian cell cycle}},
    year = {2006}
}

@book{Gardiner_2004,
    author = {Gardiner, C.},
    publisher = {Springer Berlin, Heidelberg},
    title = {{Handbook of Stochastic Methods}},
    year = {2004}
}

@article{Gardner_2000,
    author = {Gardner, T. S. and Cantor, C. R. and Collins, J. J.},
    doi = {10.1038/35002131},
    journal = {Nature},
    volume = {403},
    pages = {339--342},
    title = {{Construction of a genetic toggle switch in \textit{Escherichia coli}}},
    year = {2000}
}

@article{Garg_2008,
    author = {Garg, A. and Di Cara, A. and Xenarios, I. and Mendoza, L. and De Micheli, G.},
    doi = {10.1093/bioinformatics/btn336},
    journal = {Bioinformatics},
    volume = {24},
    number = {17},
    pages = {1917--1925},
    title = {{Synchronous versus asynchronous modeling of gene regulatory networks}},
    year = {2008}
}

@article{Gaudet_2012,
    author = {Gaudet, S. and Spencer, S. L. and Chen, W. W. and Sorger, P. K.},
    doi = {10.1371/journal.pcbi.1002482},
    journal = {PLOS Comput. Biol.},
    volume = {4},
    number = {8},
    title = {{Exploring the Contextual Sensitivity of Factors that Determine Cell-to-Cell Variability in Receptor-Mediated Apoptosis}},
    year = {2012}
}

@article{Gillespie_1976,
    author = {Gillespie, D. T.},
    doi = {10.1016/0021-9991(76)90041-3},
    journal = {J. Comput. Phys.},
    volume = {22},
    number = {4},
    pages = {403--434},
    title = {{A general method for numerically simulating the stochastic time evolution of coupled chemical reactions}},
    year = {1976}
}

@article{Gillespie_1977,
    author = {Gillespie, D. T.},
    doi = {10.1021/j100540a008},
    journal = {J. Chem. Phys.},
    volume = {81},
    number = {25},
    pages = {2340–-2361},
    title = {{Exact stochastic simulation of coupled chemical reactions}},
    year = {1977}
}

@article{Gillespie_1992,
    author = {Gillespie, D. T.},
    doi = {10.1016/0378-4371(92)90283-V},
    journal = {Physica A},
    volume = {188},
    number = {1},
    pages = {404--425},
    title = {{A rigorous derivation of the chemical master equation}},
    year = {1992}
}

@article{Gillespie_2000,
    author = {Gillespie, D. T.},
    doi = {10.1063/1.481811},
    journal = {J. Chem. Phys.},
    volume = {113},
    pages = {297--306},
    title = "{{The chemical Langevin equation}}",
    year = {2000}
}

@article{Gillespie_2001,
    author = {Gillespie, D. T.},
    doi = {10.1063/1.1378322},
    journal = {J. Chem. Phys.},
    volume = {115},
    number = {4},
    pages = {1716--1733},
    title = "{{Approximate accelerated stochastic simulation of chemically reacting systems}}",
    year = {2001}
}

@InProceedings{Gong_2011,
    author = {Gong, H. and Wang, Q. and Zuliani, P. and Faeder, J. and Lotze, M. and Clarke, E.},
    editor = {Al-Mubaid, H.},
    pages = {245--250},
    booktitle = {{Proceedings of the ISCA 3rd International Conference on Bioinformatics and Computational Biology 2011 (BICoB-2011)}},
    title = {{Symbolic Model Checking of Signaling Pathways in Pancreatic Cancer}},
    year = {2011},
    publisher = {ISCA}
}

@article{Grieco_2013,
    author = {Grieco, L. and Calzone, L. and Bernard-Pierrot, I. and Radvanyi, F. and Kahn-Perl\`{e}s, B. and Thieffry, D.},
    doi = {10.1371/journal.pcbi.1003286},
    journal = {PLOS Comput. Biol.},
    volume = {9},
    number = {10},
    title = {{Integrative Modelling of the Influence of MAPK Network on Cancer Cell Fate Decision}},
    year = {2013}
}

@article{Grima_2008,
    author = {Grima, R. and Schnell, S.},
    doi = {10.1042/bse0450041},
    journal = {Essays Biochem.},
    volume = {45},
    pages = {41--56},
    title = {{Modelling reaction kinetics inside cells}},
    year = {2008}
}

@misc{Guennebaud_2010,
    author = {Guennebaud, G. and Jacob, B. and others},
    title = {Eigen v3},
    url = {http://eigen.tuxfamily.org},
    year = {2010}
}

@article{Guo_2024,
    author = {Guo, W. and Qiu, J.-M.},
    doi = {10.1137/22M1473960},
    journal = {SIAM J. Sci. Comput.},
    volume = {46},
    number = {1},
    pages = {A232--A263},
    title = {{A conservative low rank tensor method for the Vlasov dynamics}},
    year = {2024}
}

@InProceedings{Hagberg_2008,
    author = {Hagberg, A. A. and Schult, D. A. and Swart, P. J.},
    editor = {Varoquaux, G. and Vaught, T. and Millman, J.},
    doi = {10.25080/TCWV9851},
    pages = {11--15},
    booktitle = {{Proceedings of the 7th Python in Science Conference (SciPy2008)}},
    title = {{Exploring network structure, dynamics, and function using \texttt{NetworkX}}},
    year = {2008}
}

@article{Harris_2006,
    author = {Harris, L. A. and Clancy, P.},
    doi = {10.1063/1.2354085},
    journal = {J. Chem. Phys.},
    volume = {125},
    number = {14},
    title = {A ``partitioned leaping'' approach for multiscale modeling of chemical reaction dynamics},
    year = {2006}
}

@article{Hegland_2007,
    author = {Hegland, M. and Burden, C. and Santoso, L. and MacNamara, S. and Booth, H.},
    doi = {10.1016/j.cam.2006.02.053},
    journal = {J. Comput. Appl. Math.},
    volume = {205},
    pages = {708--724},
    title = {{A solver for the stochastic master equation applied to gene regulatory networks}},
    year = {2007}
}

@article{Hegland_2008,
    author = {Hegland, M. and Hellander, A. and L\"{o}tstedt, P.},
    doi = {10.1007/s10543-008-0174-z},
    journal = {BIT Numer. Math.},
    volume = {48},
    pages = {265--283},
    title = {{Sparse grids and hybrid methods for the chemical master equation}},
    year = {2008}
}

@article{Hegland_2011,
    author = {Hegland, M. and Garcke, J.},
    doi = {10.21914/anziamj.v52i0.3895},
    journal = {ANZIAM J.},
    volume = {52},
    pages = {C628--C643},
    title = {{On the numerical solution of the chemical master equation with sums of rank one tensors}},
    year = {2011}
}

@InProceedings{Henzinger_2009,
    author = {Henzinger, T. A. and Mateescu, M. and Wolf, V.},
    editor = {Bouajjani, A. and Maler, O.},
    doi = {10.1007/978-3-642-02658-4_27},
    volume = {5643},
    pages = {337--352},
    series = {LNTCS 5643},
    booktitle = {{Computer Aided Verification}},
    title = {{Sliding Window Abstraction for Infinite Markov Chains}},
    year = {2009},
    publisher = {Springer}
}

@article{Ion_2021,
    author = {Ion, I. G. and Wildner, C. and Loukrezis, D. and Koeppl, H. and De Gersem, H.},
    doi = {10.1063/5.0045521},
    journal = {J. Chem. Phys.},
    volume = {155},
    number = {034102},
    title = {{Tensor-train approximation of the chemical master equation and its application for parameter inference}},
    year = {2021}
}

@Misc{Jacob_2006,
    author = {Jacob, B. and Guennebaud, G.},
    title = {{Eigen}},
    howpublished = {\url{http://gts.sourceforge.net/}},
    year = {2006--2021}
}

@article{Jahnke_2007,
    author = {Jahnke, T. and Huisinga, W.},
    doi = {10.1007/s00285-006-0034-x},
    journal = {J. Math. Biol.},
    volume = {54},
    pages = {1--26},
    title = {Solving the chemical master equation for monomolecular reaction systems analytically},
    year = {2007}
}

@article{Jahnke_2008,
    author = {Jahnke, T. and Huisinga, W.},
    doi = {10.1007/s11538-008-9346-x},
    journal = {Bull. Math. Biol.},
    volume = {70},
    pages = {2283--2302},
    title = {{A Dynamical Low-Rank Approach to the Chemical Master Equation}},
    year = {2008}
}

@article{Jahnke_2010,
    author = {Jahnke, T. and Udrescu, T.},
    doi = {10.1016/j.jcp.2010.04.015},
    journal = {J. Comput. Phys.},
    volume = {229},
    pages = {5724--5741},
    title = {Solving chemical master equations by adaptive wavelet compression},
    year = {2010}
}

@article{Jahnke_2010a,
    author = {Jahnke, T.},
    doi = {10.1137/080742324},
    journal = {SIAM J. Sci. Comput.},
    volume = {31},
    number = {6},
    pages = {4373--4394},
    title = {An adaptive wavelet method for the chemical master equation},
    year = {2010}
}

@article{VanKampen_1976,
    author = {Van Kampen, N. G.},
    doi = {10.1016/0375-9601(76)90398-4},
    journal = {Phys. Lett. A},
    volume = {59},
    number = {5},
    pages = {333--334},
    title = {{The equilibrium distribution of a chemical mixture}},
    year = {1976}
}

@book{VanKampen_2007,
    author = {Van Kampen, N. G.},
    doi = {10.1016/B978-0-444-52965-7.X5000-4},
    publisher = {North Holland},
    title = {{Stochastic Processes in Physics and Chemistry}},
    year = {2007}
}

@article{Kauffman_1969,
    author = {Kauffman, S. A.},
    doi = {10.1016/0022-5193(69)90015-0},
    journal = {J. Theoret. Biol.},
    volume = {22},
    pages = {437--467},
    title = {{Metabolic Stability and Epigenesis in Randomly Constructed Genetic Nets}},
    year = {1969}
}

@article{Kazeev_2014,
    author = {Kazeev, V. and Khammash, M. and Nip, M. and Schwab, C.},
    doi = {10.1371/journal.pcbi.1003359},
    journal = {PLOS Comput. Biol.},
    volume = {10},
    number = {3},
    title = {{Direct Solution of the Chemical Master Equation Using Quantized Tensor Trains}},
    year = {2014}
}

@article{Kazeev_2015,
    author = {Kazeev, V. and Schwab, C.},
    doi = {10.1137/130927218},
    journal = {SIAM J. Matrix Anal. Appl.},
    volume = {36},
    number = {3},
    pages = {1221--1247},
    title = {{Tensor approximation of stationary distributions of chemical reaction networks}},
    year = {2015}
}

@article{Kernighan_1970,
    author = {Kernighan, B. W. and Lin, S.},
    doi = {10.1002/j.1538-7305.1970.tb01770.x},
    journal = {Bell Labs Tech. J.},
    volume = {49},
    number = {2},
    pages = {291--307},
    title = {{An efficient heuristic procedure for partitioning graphs}},
    year = {1970}
}

@article{Kieri_2016,
    author = {Kieri, E. and Lubich, C. and Walach, H.},
    doi = {10.1137/15M1026791},
    journal = {SIAM J. Numer. Anal.},
    volume = {54},
    number = {2},
    pages = {1020--1038},
    title = {{Discretized dynamical low-rank approximation in the presence of small singular values}},
    year = {2016}
}

@article{Koch_2007,
    author = {Koch, O. and Lubich, C.},
    doi = {10.1137/050639703},
    journal = {SIAM J. Matrix Anal. Appl.},
    volume = {29},
    number = {2},
    pages = {434--454},
    title = {{Dynamical Low-Rank Approximation}},
    year = {2007}
}

@article{Kormann_2015,
    author = {Kormann, K.},
    doi = {10.1137/140971270},
    journal = {SIAM J. Sci. Comput.},
    volume = {37},
    pages = {613--632},
    title = {{A semi-Lagrangian Vlasov solver in tensor train format}},
    year = {2015}
}

@article{Kurtz_1972,
    author = {Kurtz, T. G.},
    doi = {10.1063/1.1678692},
    journal = {Journal of Chemical Physics},
    volume = {57},
    pages = {2976--2978},
    title = {{The Relationship between Stochastic and Deterministic Models for Chemical Reactions}},
    year = {1972}
}

@article{Kusch_2021,
    author = {Kusch, J. and Stammer, P.},
    doi = {10.1051/m2an/2022090},
    journal = {ESAIM: Math. Model. Numer. Anal.},
    volume = {57},
    number = {2},
    pages = {865--891},
    title = {{A robust collision source method for rank adaptive dynamical low-rank approximation in radiation therapy}},
    year = {2023}
}

@article{Kusch_2022,
    author = {Kusch, J. and Whewell, B. and McClarren, R. and Frank, M.},
    doi = {10.1016/j.jcp.2022.111587},
    journal = {J. Comput. Phys.},
    volume = {470},
    number = {111587},
    title = {{A low-rank power iteration scheme for neutron transport critically problems}},
    year = {2022}
}

@article{Kusch_2023,
    author = {Kusch, J. and Einkemmer, L. and Ceruti, G.},
    doi = {10.1137/21m1446289},
    journal = {SIAM J. Sci. Comput.},
    volume = {45},
    number = {1},
    pages = {A1--A24},
    title = {{On the Stability of Robust Dynamical Low-Rank Approximations for Hyperbolic Problems}},
    year = {2023}
}

@article{Kusch_2024,
    author = {Kusch, J.},
    doi = {10.48550/arXiv.2403.02834},
    journal = {arXiv},
    title = {{Second-order robust parallel integrators for dynamical low-rank approximation}},
    year = {2024}
}

@article{Li_2004,
    author = {Li, F. and Long, T. and Lu, Y. and Ouyang, Q. and Tang, C.},
    doi = {10.1073/pnas.0305937101},
    journal = {PNAS},
    volume = {101},
    number = {14},
    pages = {4781--4786},
    title = {{The yeast cell-cycle network is robustly designed}},
    year = {2004}
}

@article{Liang_2012,
    author = {Liang, J. and Han, J.},
    doi = {10.1186/1752-0509-6-113},
    journal = {BMC Syst. Biol.},
    volume = {6},
    number = {113},
    title = {{Stochastic Boolean networks: An efficient approach to modeling gene regulatory networks}},
    year = {2012}
}

@article{Lopez_2013,
    author = {Lopez, C. F. and Muhlich, J. L. and Bachman, J. A. and Sorger, P. K.},
    doi = {10.1038/msb.2013.1},
    journal = {Mol. Syst. Biol.},
    volume = {9},
    number = {1},
    pages = {646},
    title = {{Programming biological models in Python using PySB}},
    year = {2013}
}

@book{Lubich_2008,
    author = {Lubich, C.},
    doi = {10.4171/067},
    title = {{From quantum to classical molecular dynamics: reduced models and numerical analysis}},
    year = {2008},
    publisher = {European Mathematical Society}
}

@article{Lubich_2013,
    author = {Lubich, C. and Rohwedder, T. and Schneider, R. and Vandereycken, B.},
    doi = {10.1137/120885723},
    journal = {SIAM J. Matrix Anal. Appl.},
    volume = {34},
    number = {2},
    pages = {470--494},
    title = {Dynamical approximation by hierarchical {T}ucker and tensor-train tensors},
    year = {2013}
}

@article{Lubich_2014,
    author = {Lubich, C. and Oseledets, I. V.},
    doi = {10.1007/s10543-013-0454-0},
    journal = {BIT Numer. Math.},
    volume = {54},
    number = {1},
    pages = {171--188},
    title = {{A projector-splitting integrator for dynamical low-rank approximation}},
    year = {2014}
}

@article{Lubich_2018,
    author = {Lubich, C. and Vandereycken, B. and Walach, H.},
    doi = {10.1137/17M1146889},
    journal = {SIAM J. Numer. Anal.},
    volume = {56},
    number = {3},
    pages = {1273--1290},
    title = {{Time Integration of Rank-Constrained Tucker Tensors}},
    year = {2018}
}

@article{MacNamara_2008,
    author = {MacNamara, S. and Burrage, K. and Sidje, R. B.},
    doi = {10.1137/060678154},
    journal = {SIAM Multiscale Model. Simul.},
    volume = {6},
    number = {4},
    pages = {1146--1168},
    title = {{Multiscale Modeling of Chemical Kinetics via the Master Equation}},
    year = {2008}
}

@article{Mai_2009,
    author = {Mai, Z. and Liu, H.},
    doi = {10.1016/j.jtbi.2009.04.024},
    journal = {J. Theor. Biol.},
    volume = {259},
    pages = {760--769},
    title = {{Boolean network-based analysis of the apoptosis network: Irreversible apoptosis and stable surviving}},
    year = {2009}
}

@article{Matthew_2023,
    author = {Matthew, S. and Carter, F. and Cooper, J. and Dippel, M. and Green, E. and Hodges, S. and Kidwell, M. and Nickerson, D. and Rumsey, B. and Reeve, J. and Petzold, L. R. and Sanft, K. R. and Drawert, B.},
    journal = {Lett. Biomath.},
    volume = {10},
    number = {1},
    pages = {87--103},
    title = {{GillesPy2: A Biochemical Modeling Framework for Simulation Driven Biological Discovery}},
    year = {2023}
}

@article{Meyer_1990,
    author = {Meyer, H.-D. and Manthe, U. and Cederbaum, L. S.},
    doi = {10.1016/0009-2614(90)87014-I},
    journal = {Chem. Phys. Letters},
    volume = {165},
    pages = {73--78},
    title = {The multi-configurational time-dependent {H}artree approach},
    year = {1990},
}

@book{Meyer_2009,
    author = {Meyer, H.-D. and Gatti, F. and Worth, G. A.},
    doi = {10.1002/9783527627400},
    title = {Multidimensional quantum dynamics},
    publisher = {John Wiley \& Sons},
    year = {2009}
}

@article{Munsky_2006,
    author = {Munsky, B. and Khammash, M.},
    doi = {10.1063/1.2145882},
    journal = {J. Chem. Phys.},
    volume = {124},
    number = {4},
    pages = {044104},
    title = {The finite state projection algorithm for the solution of the chemical master equation},
    year = {2006}
}

@article{Niarakis_2021,
    author = {Niarakis, A. and Helikar, T.},
    doi = {10.1093/bib/bbaa236},
    journal = {Brief. Bioinform.},
    volume = {22},
    number = {4},
    pages = {1--19},
    title = {A practical guide to mechanistic systems modeling in biology using a logic-based approach},
    year = {2021}
}

@article{Nicholson_2023,
    author = {Nicholson, S. B. and Gingrich, T. R.},
    doi = {10.1103/PhysRevX.13.041006},
    journal = {Phys. Rev. X},
    volume = {13},
    number = {041006},
    title = {{Quantifying Rare Events in Stochastic Reaction-Diffusion Dynamics Using Tensor Networks}},
    year = {2023}
}

@article{Niepel_2009,
    author={Niepel, M. and Spencer, S. L. and Sorger, P. K.},
    doi = {10.1016/j.cbpa.2009.09.015},
    volume = {13},
    number = {5-6},
    pages = {556--561},
    title = {{Non-genetic cell-to-cell variability and the consequences for pharmacology}},
    journal = {Curr. Opin. Chem. Biol.},
    year = {2009}
}

@article{Nguyen_2016,
    author = {Nguyen, L. K. and Kholodenko, B. N.},
    doi = {10.1016/j.semcdb.2015.09.024},
    journal = {Seminar in Cell \& Developmental Biology},
    volume = {50},
    pages = {85--94},
    title = {{Feedback regulation in cell signalling: Lessons for cancer therapeutics}},
    year = {2016}
}

@article{LeNovere_2015,
    author = {Le Nov\`{e}re, N.},
    doi = {10.1038/nrg3885},
    journal = {Nat. Rev. Genet.},
    volume = {16},
    pages = {146--158},
    title = {{Quantitative and logic modelling of molecular and gene networks}},
    year = {2015}
}

@article{Paszek_2010,
    author = {Paszek, P. and Ryan, S. and Ashall, L. and Sillitoe, K. and Harper, C. V. and Spiller, D. G. and Rand, D. A. and White, M. R.H.},
    doi = {10.1073/pnas.0913798107},
    journal = {PNAS},
    volume = {107},
    number = {25},
    pages = {11644--11649},
    title = {{Population robustness arising from cellular heterogeneity}},
    year = {2010}
}

@article{Peng_2020,
    author = {Peng, Z. and McClarren, R. and Frank, M.},
    doi = {10.1016/j.jcp.2020.109735},
    journal = {J. Comput. Phys.},
    volume = {421},
    number = {109735},
    title = {{A low-rank method for two-dimensional time-dependent radiation transport calculations}},
    year = {2020}
}

@article{Peng_2021,
    author = {Peng, Z. and McClarren, R.},
    doi = {10.1016/j.jcp.2021.110672},
    journal = {J. Comput. Phys.},
    volume = {447},
    number = {110672},
    title = {{A high-order/low-order (HOLO) algorithm for preserving conservation in time-dependent low-rank transport calculations}},
    year = {2021}
}

@article{Pino_2020,
    author = {Pino, J. C. and Prugger, M. and Lubbock, A. L. R. and Harris, L. A. and Lopez, C. F.},
    doi = {10.1101/2020.02.14.948612},
    journal = {bioRxiv},
    title = {{Accelerated Simulations of Chemical Reaction Systems using the Stochastic Simulation Algorithm on GPUs}},
    year = {2020}
}

@article{Prugger_2021,
    author = {Prugger, M. and Einkemmer, L. and Beik, S. P and Wasdin, P. T. and Harris, L. A. and Lopez, C. F.},
    doi = {10.1371/journal.pcbi.1009035},
    journal = {PLOS Comput. Biol.},
    volume = {17},
    number = {6},
    title = {{Unsupervised logic-based mechanism inference for network-driven biological processes}},
    year = {2021}
}

@article{Prugger_2023,
    author = {Prugger, M. and Einkemmer, L. and Lopez, C. F.},
    doi = {10.1016/j.jcp.2023.112250},
    journal = {J. Comput. Phys.},
    volume = {489},
    page = {112250},
    title = {{A dynamical low-rank approach to solve the chemical master equation for biological reaction networks}},
    year = {2023}
}

@article{Raj_2008,
    author = {Raj, A. and Van Oudenaarden, A.},
    doi = {10.1016/j.cell.2008.09.050},
    journal = {Cell},
    volume = {135},
    number = {2},
    page = {216--226},
    title = {{Nature, Nurture, or Chance: Stochastic Gene Expression and Its Consequences}},
    year = {2008}
}

@article{Reis_2018,
    author = {Reis, M. and Kromer, J. A. and Klipp, E.},
    doi = {10.1007/s00285-018-1205-2},
    journal = {J. Math. Biol.},
    volume = {77},
    pages = {377--419},
    title = {General solution of the chemical master equation and modality of marginal distributions for hierarchic first-order reaction networks},
    year = {2018}
}

@article{Ribeiro_2006,
    author = {Ribeiro, A. and Zhu, R. and Kauffman, S. A.},
    doi = {10.1089/cmb.2006.13.1630 },
    journal = {J. Comput. Biol.},
    volume = {13},
    number = {9},
    pages = {1630--1639},
    title = {{A General Modeling Strategy for Gene Regulatory Networks with Stochastic Dynamics}},
    year = {2006}
}

@article{Saad_1986,
    author = {Saad, Y. and Schultz, M. H.},
    doi = {10.1137/0907058},
    journal = {SIAM J. Sci. Stat. Comput.},
    volume = {7},
    number = {3},
    title = {{GMRES: A generalized minimal residual algorithm for solving nonsymmetric linear systems}},
    year = {1986}
}

@article{Samoilov_2006,
    author = {Samoilov, M. S. and Arkin, A. P.},
    doi = {10.1038/nbt1253},
    journal = {Nat. Biotechnol.},
    volume = {24},
    number = {10},
    pages = {1235--1240},
    title = {{Deviant effects in molecular reaction pathways}},
    year = {2006}
}

@article{Sanft_2011,
    author = {Sanft, K. R. and Wu, S. and Roh, M. and Fu, J. and Lim, R. K. and Petzold, L. R.},
    doi = {10.1093/bioinformatics/btr401},
    journal = {Bioinformatics},
    volume = {27},
    number = {17},
    pages = {2457--2458},
    title = {{StochKit2: software for discrete stochastic simulation of biochemical systems with events}},
    year = {2011}
}

@article{Schloegl_1971,
    author = {Schl\"{o}gl, F.},
    doi = {doi.org/10.1007/BF01395694},
    journal = {Z. Physik},
    volume = {248},
    pages = {446--458},
    title = {On thermodynamics near a steady state},
    year = {1971}
}

@article{Shannon_1948,
    author = {Shannon, C. E.},
    doi = {10.1002/j.1538-7305.1948.tb01338.x},
    journal = {Bell Syst. Tech. J.},
    volume = {27},
    number = {3},
    pages = {379--423},
    title = {{A Mathematical Theory of Communication}},
    year = {1948}
}

@article{Shmulevich_2002,
    author = {Shmulevich, I. and Dougherty, E. R. and Kim, S. and Zhang, W.},
    doi = {10.1093/bioinformatics/18.2.261},
    journal = {Bioinformatics},
    volume = {18},
    number = {2},
    pages = {261--274},
    title = {{Probabilistic Boolean networks: a rule-based uncertainty model for gene regulatory networks}},
    year = {2002}
}

@article{Stoll_2012,
    author = {Stoll, G. and Viara, E. and Barillot, E. and Calzone, L.},
    doi = {10.1186/1752-0509-6-116},
    journal = {BMC Syst. Biol.},
    volume = {6},
    number = {116},
    title = {{Continuous time boolean modeling for biological signaling: application of Gillespie algorithm}},
    year = {2012}
}

@article{Sulz_2024,
    author = {Sulz, D. and Lubich, C. and Ceruti, G. and Lesanovsky, I. and Carollo, F.},
    doi = {10.1103/PhysRevA.109.022420},
    journal = {Phys. Rev. A},
    volume = {109},
    number = {022420},
    title = {{Numerical simulation of long-range open quantum many-body dynamics with tree tensor networks}},
    year = {2024}
}

@article{Thomas_1973,
    author = {Thomas, R.},
    doi = {10.1016/0022-5193(73)90247-6},
    journal = {J. Theor. Biol.},
    volume = {42},
    number = {3},
    pages = {563--585},
    title = {{Boolean formalization of genetic control circuits}},
    year = {1973}
}

@article{Thomas_1991,
    author = {Thomas, R.},
    doi = {10.1016/S0022-5193(05)80350-9},
    journal = {J. Theor. Biol.},
    volume = {153},
    number = {1},
    pages = {1--23},
    title = {{Regulatory Networks Seen as Asynchronous Automata: A Logical Description}},
    year = {1991}
}

@article{Tonn_2019,
    author = {Tonn, M. K. and Thomas, P. and Barahona, M. and Oyarz\'{u}n, D. A.},
    doi = {10.1038/s42003-019-0347-0},
    journal = {Commun. Biol.},
    volume = {2},
    number = {108},
    title = {{Stochastic modelling reveals mechanisms of metabolic heterogeneity}},
    year = {2019}
}

@article{Vahedi_2009,
    author = {Vahedi, G. and Faryabi, B. and Chamberland, J.-F. and Datta, A. and Dougherty, E. R.},
    doi = {10.1016/j.jtbi.2009.08.026},
    journal = {J. Theoret. Biol.},
    volume = {261},
    pages = {540--547},
    title = {{Sampling-rate-dependent probabilistic Boolean networks}},
    year = {2009}
}

@article{Wang_2012,
    author = {Wang, R.-S. and Saadatpour, A. and Albert, R.},
    doi = {10.1088/1478-3975/9/5/055001},
    journal = {Phys. Biol.},
    volume = {9},
    number = {055001},
    title = {Boolean modeling in systems biology: an overview of methodology and applications},
    year = {2012}
}

@article{Wolf_2010,
    author = {Wolf, V. and Goel, R. and Mateescu, M. and Henzinger, T. A.},
    doi = {10.1186/1752-0509-4-42},
    journal = {BMC Syst. Biol.},
    volume = {4},
    number = {42},
    title = {Solving the chemical master equation using sliding windows},
    year = {2010}
}

@article{Yachie-Kinoshita_2018,
    author = {Yachie-Kinoshita, A. and Onishi, K. and Ostblom, J. and Langley, M. A. and Posfai, E. and Rossant, J. and Zandstra, P. W.},
    doi = {10.15252/msb.20177952},
    journal = {Mol. Syst. Biol.},
    volume = {14},
    number = {1},
    title = {{Modeling signaling-dependent pluripotency with Boolean logic to predict cell fate transitions}},
    year = {2018}
}

@article{Ye_2023,
    author = {Ye, E. and Loureiro, N. F.},
    doi = {10.48550/arXiv.2311.07756},
    journal = {arXiv},
    title = {{Quantized tensor networks for solving the Vlasov--Maxwell equations}},
    year = {2023}
}

@article{Zanudo_2018,
    author = {Za\~{n}udo, J. G. T. and Steinway, S. N. and R\'{e}ka, A.},
    doi = {10.1016/j.coisb.2018.02.002},
    journal = {Curr. Opin. Syst. Biol.},
    volume = {9},
    pages = {1--10},
    title = {{Discrete dynamic network modeling of oncogenic signaling: Mechanistic insights for personalized treatment of cancer}},
    year = {2018}
}
